Reenactment for Read-Committed Snapshot Isolation

Provenance for transactional updates is critical for many applications such as auditing and debugging of transactions. Recently, we have introduced MV-semirings, an extension of the semiring provenance model that supports updates and transactions. Furthermore, we have proposed reenactment, a declarative form of replay with provenance capture, as an efficient and non-invasive method for computing this type of provenance. However, this approach is limited to the snapshot isolation (SI) concurrency control protocol while many real world applications apply the read committed version of snapshot isolation (RC-SI) to improve performance at the cost of consistency. We present non-trivial extensions of the model and reenactment approach to be able to compute provenance of RC-SI transactions efficiently. In addition, we develop techniques for applying reenactment across multiple RC-SI transactions. Our experiments demonstrate that our implementation in the GProM system supports efficient re-construction and querying of provenance.

==> background.tex <==
\section{Snapshot Isolation} %Read Committed
\label{sec:background}

%\BG{We also need some part on snapshot isolation for the readers that do not know what snapshot isolation is}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Snapshot Isolation}
% \label{sec:snapshot-isolation}

Snapshot isolation (SI)~\cite{JB95,BB95} is a widely applied multi-versioning
concurrency control protocol. Under SI each trans\-ac\-tion $\xid$ sees a private
snapshot of the database containing changes of transactions that have committed
before $\xid$ started and $\xid$'s own changes. Using SI, reads do never block
concurrent reads and writes, because each transaction sees a consistent version
of the database as of its start (and, as mentioned before, its own changes). To
support such snapshots, old versions of tuples cannot be removed until all
transactions that may need them have finished. Typically, this is implemented by
storing multiple timestamped versions of each tuple and assigning a timestamp to
every transaction when it begins that determines which version of the database
this transaction will see (its snapshot). Whether a certain version of a tuple
is visible to a transaction can be checked by comparing its timestamp (if it is
a committed tuple version) with the transaction's timestamp.

Concurrent writes are allowed under SI. However, if several concurrent
transactions have written the same data item, only one of them will be allowed
to commit. There are several ways how to enforce this constraint. Most systems implementing this protocol use write locks to block transactions from writing the same data item. A transaction waiting for a write lock has to abort if the transaction currently holding the lock commits and acquires the lock if the transaction holding the lock aborts.

% One option is
% to check at commit time for transaction $\xid$ whether any concurrent
% transaction has an overlapping write set (has modified a data item written by
% transaction $\xid$). 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Read Committed Snapshot Isolation}
% \label{sec:stat-level-snapsh}

Database systems implementing SI as a concurrency control protocol typically also support
a variant of SI with statement-level snapshots as a substitute for the standard
\texttt{READ COM\-MIT\-TED} isolation level. As mentioned before, we refer to this protocol as
\textit{read committed snapshot isolation} (\textit{RC-SI}). Under RC-SI each
statement of a transaction sees changes of transactions that committed before the
statement was executed. In contrast to SI, transactions waiting for a write lock
are allowed to resume their operation once the lock is released no matter
whether the transaction holding this lock committed or aborted. The exact
details of the implementation differ from system to system. For instance, Oracle
restarts an update that had to wait for a write lock to guarantee that the
updates sees a consistant snapshot of the database. In contrast, in PostgreSQL
the update is resumed after the lock it is waiting for is released. In this
paper we assume the RC-SI semantics implemented by Oracle.

% \begin{itemize}
% \item Each statement sees consistent snapshot
%   \begin{itemize}
%   \item It sees data committed by transactions before the statement began
%   \item It sees changes made by previous statements of the same transaction
%   \end{itemize}
% \item If a statements waits for a write lock it either continues if the transaction holding the lock aborts or 
% \item 
% \end{itemize}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
%   \centering
  
%   \begin{tabular}{|cc|}
%     \thead{Semiring} & \thead{Corresponding Model} \\
%     $(\mathbb{B}, \vee, \wedge, false, true)$ & Set semantics\\
%     $(\mathbb{N}, +, \times, 0, 1)$ & Bag semantics\\
%     $({\cal P}(X) \union \{\perp\}, \union_+, \union_\times, \perp, \emptyset)$ & Lineage\\
%     $(\ppSR, +, \times, 0, 1)$ & Provenance polynomials\\ \hline
%   \end{tabular}

%   \caption{Example Semiring}
%   \label{fig:example-SR}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{Should we maybe directly introduce our model for SI and update annotations directly alongside with the Semiring framework?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theo}[Snapshots Commute With Queries]
  
% \end{theo}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This semantics has been shown to
% generalize several extensions of the relational model including
% bag-semantics, incomplete databases, and several provenance
% models. The authors have demonstrated that the

% \begin{itemize}
% \item Introduce some semirings
% \item Motivate what $+$ and $\times$ means: conjunctive and
%   disjunctive use of tuples
% \item Motivate that provenance polynomials generalize all other semirings
% \end{itemize}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "rc_reenactment"
%%% End: 


==> optimizations.tex <==

\section{Optimizations}
\label{sec:optimize}
We applied some heuristic optimization techniques. We review some of them in Appendix~\ref{sec:Optimizations}.

\subsection{Unique Solution for RC-SI Transactions}
\label{sec:updated-only}

We applied a unique solution and likely more efficient way to chain the updates of RC-SI transaction. We know that tuples versions committed in between $R^0$ and $R^c$ have been seen by at least on $u_i$ from $T$. Let $k$ be the newest version of $t$ in the interval $[0,c]$, then apparently no update $u_j$ with $j < k$ from transaction $T$ has updated $t$. Thus, for these updates we do not need to check whether $t$ would be updated. We get $R^{c-1}$ and add a version column $V$ that is produced by mapping the SCN of each tuple to an update $u_j$ from $T$  as follows: $V$ is set to $i$ if the time of $t$'s last modification falls in the interval $[t_{i-1}, t_{i}]$. Let $R^{*}$ denote the result of this operation. We let $q(u_0)$ read from $R^*$ directly. The update translation $q(u_i)$ is modified by changing the condition for the update branch of $u_i$ to $C_i \wedge V \leq i$ and for the non-update branch to $\neg C_i \vee V > i$. The projection for the update branch is modified to set $V = i$. In this translation each update query translation is reading from the previous update's query translation. Alternatively, we may use the SCN of tuples directly to spare the version computation at the cost of more complex selection conditions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{exam}
For the second translation scheme consider an transaction $T$ over table $R$ shown below. Let $SCN(u_i)$ denote the SCN of update statement $u_i$.

\begin{minipage}{1.0\linewidth}
  \centering
  \begin{tabular}{c|c}
    A & B\\ \hline
    2 & 5 \\
    10 & 3\\
    11 & 4\\
  \end{tabular}
\end{minipage}

\begin{lstlisting}
$u_0$: UPDATE R SET a = a + 2 WHERE b = 5;
$u_1$: UPDATE R SET a = a + 5 WHERE b = 3;
$c_1$: COMMIT;
\end{lstlisting}

Lets assume that between $u_0$ and $u_1$ a second transaction $T'$ executes the following update and commits:

\begin{lstlisting}
$u_a$: UPDATE R SET a = -1 WHERE b = 3;
\end{lstlisting}

Assume the SCNs are $SCN(u_0) = 19, SCN(u_1) = 37, \\
SCN(u_a) = 28$. Then we first create $R^*$:

\begin{lstlisting}
WITH Rstart AS
SELECT a, b, 
    CASE 
      WHEN VERSIONS_STARTSCN <= 19 
      	OR VERSIONS_STARTSCN IS NULL THEN 0 
      WHEN VERSIONS_STARTSCN > 19
      	AND VERSIONS_STARTSCN < 37 THEN 1
      ELSE -1
    END AS version_
FROM R VERSIONS BETWEEN SCN 36 AND 36
\end{lstlisting}

Then the translated updates (using the case method) is (getting only back updated tuples):

\begin{lstlisting}
u0 AS     
     (SELECT
           CASE WHEN b = 5 AND version_ <= 0 
           	THEN a + 2 ELSE a END AS a,
           b,
           CASE WHEN b = 5 AND version_ <= 0 THEN
           	 -1 ELSE version_ END AS version_
     FROM Rstar) 
,
u1 AS
     (SELECT
       CASE WHEN b = 5 AND version_ <= 1
       	 THEN a + 5 ELSE a END AS a,
       b,
       CASE WHEN b = 5 AND version_ <= 1 
       	THEN -1 ELSE version_ END AS version_
      FROM u0)

SELECT a,b FROM u1 WHERE version_ = -1;
\end{lstlisting}

\end{exam}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "rc_reenactment"
%%% End: 


==> rc_isolation.tex <==
\section{Read Committed Snapshot Isolation}
\label{sec:SI-prov}

Under  read  committed  snapshot isolation  (RC-SI)~\footnote{Recall  that  this
  corresponds to isolation level \lstinline!READ COMMITTED! in databases such as
  Oracle or Postgres} each update $u$  within a transaction sees changes made by
previous updates of  the same transaction and changes of  transactions that have
committed before  $u$ was  executed. Recall  that under RC-SI  each update  of a
transaction sees changes  of transactions which committed before  the update was
executed.  Thus, we  have  to  adapt the  definitions  of $R[\xid,\version]$  to
include      changes     of      concurrent     transactions.      We     define
$\relSSI{\rel}{\xid}{\version}$ which  denotes the version of  relation $R$ seen
by transaction $\xid$ at version $\version$  and thus version includes both past
changes of $\xid$ and annotations  created by transactions that committed before
$\version$.  Consider  the  range  of  the   outer  sum  in  the  definition  of
$\relSSI{\rel}{\xid}{\version}$. This sum ranges over all transactions that have
committed before $\version$ and $\xid$ itself.

\input{historic_def}

Again, we define a relation $\validAt$ which determines whether a summand in an
annotation is valid at time $\version$. However, now this validity is specific
to a transaction $\xid$.  A summand is valid if it was produced by $\xid$
itself (second row in the case distinction). In addition, it is also valid if it
was produced by transaction $\xid'$ and no other transaction that has committed
or is equal to $\xid$ has overwritten this summand.  The definition of $\hasUp$
is the same as under SI.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{defi}[RC-SI Historic Database]
  Let $\history$ be a history over a database $\db$. The history database
  $\db(\history,RC-SI)$ of $\db$ based on $\history$ is a set of historic
  relations.  $R^{\version}$ for $R$ in $\db$ is defined in
  Figure~\ref{fig:ssi-hist-db-definitions}.
\end{defi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Similar to how $\SReval$ and $\unversion$ commute with queries and updates, the
same also holds for transactions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{propo}[$\SReval$ commutes with histories]
  Let $\nu$ be a valuation from variables $X$ to elements of a MV-semiring
  $\mvK$. Then $\SReval_\nu$ and $\unversion$ commute with histories.
\end{propo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This theorem shows that we can evaluate histories using the $\ppSRV$ MV-semiring
and derive the result of applying a history in any MV-semiring from
$\history(D)$ evaluated in $\ppSRV$. However, this does not necessarily imply
that our approach correctly generalizes SI and RC-SI for set and bag
semantics. It remains to show that $\history(D)$ if evaluated under
$\mathbb{B}^{\version}$ and $\mathbb{N}^{\version}$, respectively, corresponds
to standard set and bag semantics evaluation of SI and RC-SI histories.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theo}[SI and SI-RC Correctness]
  Let $D_{\mathbb{B}}$\\ and $D_{\mathbb{N}}$ be the result of evaluating a
  history $\history$ under standard bag semantics and set semantics using SI,
  receptively. Then $D_{\mathbb{B}} = \history(D)$ if evaluated in $\mathbb{B}$
  and $D_{\mathbb{N}} = \history(D)$ if evaluated in $\mathbb{B}$. The same
  holds for RC-SI.
\end{theo}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  We have already shown that updates executed under $\mvK$ semantics correspond
  to set and bag semantics if $\mvK= \mathbb{B}$ and $\mvK = \mathbb{N}$,
  respectively. Thus, it remains to show that our definition of $\history(D)$
  obeys the visibility rules of SI and RC-SI, respectively.

\noindent\underline{\bf SI}: Under SI each update of a transaction $\xid$ sees
changes by transaction that committed before $\xid$ started and updates of
previous statements of $\xid$. For a sequence of statements within $\xid$ the
correctness follows from the correctness for single updates. It remains to show
that $\relCV{\rel}{\version}$ is correct. $\relCV{\rel}{\version}$ has to
contains all changes to relation $R$ of transactions that committed before
$\version$. Obviously, this set contains all tuple versions created by
transactions that have committed before $\version$ and that have not been
overwritten by preceding transactions which also committed before $\version$. We
prove that this set corresponds to $\relCV{\rel}{\version}$ by induction over
the number of transaction that have committed before $\version$.

\underline{Induction Start:} Per convention the initial state of the database is
empty and, thus, the conjecture trivially holds. If only a single transaction
$\xid'$ committed before $\version$ then $\relCV{\rel}{\version}$ is the result
of a single sequence update operations (the operations of transaction $\xid'$)
and the correctness follows from the correctness for simple updates.

\underline{Induction Step:} Assume that the conjecture holds for $i$ transaction
that committed before $\version$. We need to show that the same applied if $i+1$
transaction have committed before $\version$. WLOG assume that the new
transaction $\xid_{i+1}$ was the last to commit. Given that $\xid_{i+1}$
committed last, all summands created by this transaction should be in
$\relCV{\rel}{\version}$. This is the case, because $\finish{\xid_{i+1}} \leq
\version$ and, thus, $\xid_{i+1}$ is considered in the outer sum of
$\relCV{\rel}{\version}$. However, we need to show that $\validAt(\xid_{i+1}, t,
k, \version)$ evaluates to $1$ for any $t$ and $k$. For any summand created by
$\xid_{i+1}$ we know from the definition of $\relCV{R}{\version}$ that this
summand was not visible to any other transaction that committed before
$\version$. This follows from the fact that $\xid_{i+1}$ was the last
transaction to commit. For any other transaction $\xid_j$ that committed before
$\xid_j$, $\relCV{R}{\start{\xid_j}}$ the outer sum does not range over
$\xid_{i+1}$, because $\finish{\xid_{i+1}} > \start{\xid_j}$. Furthermore, we
need to show that any summand created by a transaction $\xid_j$ that was
overwritten by $\xid_{i+1}$ is not present in $\relCV{R}{\version}$. Let $k$ be
such an summand in an annotation for a tuple $t$ created by transaction $\xid_j$
with $\finish{\xid_j} < \start{\xid_{i+1}}$. Note that we do not need to
consider case $\finish{\xid_j} > \start{\xid_{i+1}}$, because annotations
created by such a transaction are not visible to $\xid_{i+1}$. WLOG assume that
transaction $\xid_{i+1}$ did overwrite $k$ using an update operation executed at
$\version' < \version$. No matter what type of update is applied (update or
delete), the result will include a summand wrapping $k$ into a version
annotation (this follows from the definition of update operations). Hence, in
$\validAt (\xid_j, t, k, \version)$ the not exists condition evaluates to false
for $\xid' = \xid_{i+1}$, because $\finish{\xid_{i+1}} < \version$ and
$\hasUp(\xid_{i+1}, t, k)$ is true. This proves the induction step.

\noindent\underline{\bf RC-SI}: The proof for RC-SI is similar in nature with
the exception that we needs to range over operations of transactions and the
visibility rules are slightly different.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "rc_reenactment"
%%% End: 



